L$_0$onie: Compressing COINs with L$_0$-constraints

Advances in Implicit Neural Representations (INR) have motivated research on domain-agnostic compression techniques. These methods train a neural network to approximate an object, and then store the weights of the trained model. For example, given an image, a network is trained to learn the mapping from pixel locations to RGB values. In this paper, we propose L$_0$onie, a sparsity-constrained extension of the COIN compression method. Sparsity allows to leverage the faster learning of overparameterized networks, while retaining the desirable compression rate of smaller models. Moreover, our constrained formulation ensures that the final model respects a pre-determined compression rate, dispensing of the need for expensive architecture search.

==> checklist.tex <==
%
\section*{Checklist}


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} Code provided in the supplementary material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See \cref{app:exp_details}.
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See \cref{app:exp_details,,app:all_comparisons}.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%

==> experiments.tex <==
\section{Achieving Controllable Sparsity}%
\label{sec:control_experiments}

In this section we revisit the learning tasks studied by \citet{louizos2017learning} and illustrate how the constrained approach affords us better interpretability and control across different architectures and datasets. We do not intend, however, to claim that constrained approaches are universally better than their penalized counterparts. Implementation details for these experiments are provided in \cref{app:exp_details}.

\subsection{Penalties vs Constraints}
\label{sec:control_mlp_lenet}
We consider a method to be \textit{controllable} if it reliably achieves a \textit{pre-specified target}. The main goal of our work is to train models that attain good predictive performance, while having a fine-grained command on their final sparsity. 

The notion of a pre-specified target is a core difference between the constrained and penalized paradigms. The lack of a pre-specified target density in the penalized formulation severely limits our ability to determine ``success" regarding the achieved density. Defining success for the constraint formulation is trivial as it only requires verifying whether the constraints are satisfied. Naturally, however, establishing the optimality of a solution remains a challenge for both approaches when faced with non-convex objectives.


Defining the pre-specified target usually requires problem-specific expertise. Consider the deployment of a (sparse) model on a resource constrained device. Ensuring low latency implies bounds on the allowed number of FLOPS, which is directly linked to the number of active parameters in the network. Thanks to the \textbf{ \textit{interpretability}} of the ``hyperparameter'' $\epsilon$ of the constrained formulation, the maximum allowed number of FLOPS can be easily translated into target density levels for (each layer of) the model. 


\cref{fig:lenet_modelwise,,fig:mlp_modelwise} show the achieved densities of WideResNets and LeNet models trained on CIFAR10/MNIST using the constrained and penalized methods. These experiments group parameters ``at the model level'': we apply a constraint or penalty, respectively, on the expected $L_0$-norm of the full model. Experimental details and results for experiments with layer-based groupings are presented in Apps. \ref{app:exp_details} and \ref{app:controllability}.

%

%
%
%
%
%
%
%
%

The behavior for LeNets closely resembles that of the WideResNet models presented in \cref{sec:introduction}. The constrained method exhibits \textbf{\textit{controllability}}: it consistently achieves the desired density across a wide span of targets. On the other hand, the sensitivity profile of the penalized method illustrates the non-trivial influence that $\lambdapen$ has on the achieved density: it is difficult to predict the shift in terms of the achieved density that would result from an arbitrary perturbation of $\lambdapen$.
We note that higher orders of magnitude for $\lambdapen$ caused training issues as the model would become completely sparse, having no active units.


\textbf{Iterative tuning.} Even in situations where a pre-specified target density is available, finding a suitable value of $\lambdapen$ which realizes this target would require running an iterative search, whose cost might be prohibitive. \cref{fig:bisection} in \cref{app:bisection} illustrates that these difficulties arise even in the simple case of MLP architectures.

%
%

%

Finally, it is worth recalling that the penalized method may not be able to recover every arbitrary constraint level \citep[$\S 4.7.4$]{boyd2004convex}.
%
%
Therefore, not only is iterative tuning computationally intensive, the ill-posedness of the problem can render it a futile search when dealing with non-convex problems.





\subsection{Sparsity Control at Test Time}
\label{sec:control_testtime}

We follow the procedure outlined in \cref{app:reparametrization} to obtain a deterministic, sparse network at test time. \cref{fig:wrn_modelwise_val} shows that the constrained method consistently delivers test time WRN models whose densities match closely the desired sparsity targets used during training. Comparisons for other architectures and parameter groupings can be found in \cref{fig:control_val} in \cref{app:controllability}.


%
%
%
%
%
%
%


%


\paragraph{Controlling the Performance-Sparsity trade-off}
\cref{fig:lenet_tradeoff} shows the trade-off profile between the achieved test time sparsity and the predictive performance of a WideResNet on CIFAR10 for the constrained and penalized methods. Trade-off profiles for the other architectures and parameter groupings can be found in \cref{fig:control_error} in \cref{app:controllability}.


The constrained method enables us to better explore the set of achievable trade-offs between sparsity and performance thanks to its control on the resulting model sparsity. In contrast, the penalized approach is highly sensitive to the value of the regularization coefficient and it results in several models with good performance, but almost no sparsity.


This observation is in line with the discussion by \citet{blog_1} on the inability of gradient descent to thoroughly explore trade-offs between linearly combined objectives for problems with non-convex Pareto frontiers.


%
%
%
%
%
%
%


\vspace*{-2ex}

\section{Performance Comparison}
\label{sec:experiments}


\task{JGP: Comparison with magnitude pruning alternative? Start both models from pre-trained to make comparison fair?}

In this section, we report the predictive test time performance of the sparse models learned using our constrained method and compare the results against the penalized approach over the same set of learning tasks studied in \citet{louizos2017learning}. Implementation details for the experiments in this section can be found in \cref{app:exp_details}.

\paragraph{MNIST} 
To ensure a fair comparison with the models obtained by \citet{louizos2017learning}, we manually calculate the achieved density levels of their reported pruned architectures and used these values as the target density levels for our approach, for both of the model- and layer-level groupings. 

\cref{tab:mnist} reports the performance levels along with the resulting pruned architecture. Note that the performance of the models learned using the constrained method is on-par with their penalized counterparts in terms of the best achieved test error. Moreover, the pruned architectures learned using the constrained approach confirm once more its beneficial controllability properties: the resulting architectures are very similar for both methods since our density targets were based on the pruned architectures of \citet{louizos2017learning}.

\paragraph{CIFAR10 and CIFAR100}
While \citet{louizos2017learning} did not report explicit sparsity metrics for WRNs, our replication of their penalized experiments resulted in no sparsity in the test time parameters. This observation was also reported by \citet{gale2019state} regarding WRNs.

\cref{tab:cifar} shows the test time performances and density levels for WRNs on the CIFAR10 and CIFAR100 datasets. By adopting the modifications detailed in \cref{sec:control_fixes}, both of the penalized and the constrained methods were able to learn sparse test time models while attaining comparable performances to those reported in \citet{louizos2017learning}.

Note how these results also confirm the qualitative controllability offered by our constrained method for WRNs. Indeed, the models trained with a $70\%$ target density successfully achieved test time densities close to this goal.

%
%

==> latex_figs/cifar100_comparison.tex <==
\begin{figure}[h!]
\setlength\tabcolsep{0pt}%
\centering
\hspace{-1.5cm}
\begin{tabular}{llccc}
 \centering
 & \hspace{2mm} & \hspace{-2mm} \textbf{$L_0$-density} & \hspace{6mm}\textbf{Parameters} & \hspace{5mm} \textbf{MACs} \\
 
\rotatebox{90}{\hspace{1.2cm} \textbf{Layer-wise}} & & \includegraphics[width=0.4\textwidth, trim={0mm 0mm 0mm 0mm}, clip]{figs/control/cifar100/ResNet-28-10_layerwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_params/cifar100/ResNet-28-10_layerwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_macs/cifar100/ResNet-28-10_layerwise.pdf} \\
\rotatebox{90}{\hspace{1.2cm} \textbf{Model-wise}} &  & \includegraphics[width=0.4\textwidth, trim={0mm 0mm 0mm 0mm}, clip]{figs/control/cifar100/ResNet-28-10_modelwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_params/cifar100/ResNet-28-10_modelwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_macs/cifar100/ResNet-28-10_modelwise.pdf} \\
\end{tabular}
    \caption[]{Training sparse WideResNet-28-10 models on CIFAR-100.}
    \label{fig:cifar100_comparison}
\end{figure}

==> latex_figs/cifar10_comparison.tex <==
\begin{figure}[h]
\vspace{-7ex}
\setlength\tabcolsep{0pt}%
\centering
\begin{tabular}{llccc}
 \centering
 & \hspace{2mm} & \hspace{-2mm} \textbf{$L_0$-density} & \hspace{6mm}\textbf{Parameters} & \hspace{5mm} \textbf{MACs} \\
 
\rotatebox{90}{\hspace{1.2cm} \textbf{Layer-wise}} & & \includegraphics[width=0.345\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/control/cifar10/ResNet-28-10_layerwise.pdf}
 & \includegraphics[width=0.27\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/error_vs_params/cifar10/ResNet-28-10_layerwise.pdf}
 & \includegraphics[width=0.27\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/error_vs_macs/cifar10/ResNet-28-10_layerwise.pdf} \\
\rotatebox{90}{\hspace{1.2cm} \textbf{Model-wise}} &  & \includegraphics[width=0.345\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/control/cifar10/ResNet-28-10_modelwise.pdf}
 & \includegraphics[width=0.27\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/error_vs_params/cifar10/ResNet-28-10_modelwise.pdf}
 & \includegraphics[width=0.27\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/error_vs_macs/cifar10/ResNet-28-10_modelwise.pdf} \\
\end{tabular}
    \caption[]{Training sparse WideResNet-28-10 models on CIFAR-10.}
    \label{fig:cifar10_comparison}
\end{figure}




==> latex_figs/dual_restarts.tex <==
\begin{figure}[h]
    \setlength\tabcolsep{0pt}%
    \centering
    %
    \includegraphics[width=0.97\textwidth]{figs/restarts/dual_restarts.pdf}
    \vspace{-1ex}
    \caption[]{Effect of dual restarts for training a LeNet5 on MNIST with a model-wise target density $\epsilon_g = 30\%$ (horizontal dashed line). The accumulation of the constraint violations in the Lagrange multiplier leads to excessive sparsification when the model satisfies the constraint. Restarting the Lagrange multiplier allows the model to concentrate on improving the training loss.}
    \label{fig:dual_restarts}
\end{figure}

==> latex_figs/mnist_lenet_comparison.tex <==
\begin{figure}[h!]
\setlength\tabcolsep{0pt}%
\centering
\hspace{-1.5cm}
\begin{tabular}{llccc}
 \centering
 & \hspace{2mm} & \hspace{-2mm} \textbf{$L_0$-density} & \hspace{6mm}\textbf{Parameters} & \hspace{5mm} \textbf{MACs} \\
 
\rotatebox{90}{\hspace{1.2cm} \textbf{Layer-wise}} & & \includegraphics[width=0.4\textwidth, trim={0mm 0mm 0mm 0mm}, clip]{figs/control/mnist/LeNet_layerwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_params/mnist/LeNet_layerwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_macs/mnist/LeNet_layerwise.pdf} \\
\rotatebox{90}{\hspace{1.2cm} \textbf{Model-wise}} &  & \includegraphics[width=0.4\textwidth, trim={0mm 0mm 0mm 0mm}, clip]{figs/control/mnist/LeNet_modelwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_params/mnist/LeNet_modelwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_macs/mnist/LeNet_modelwise.pdf} \\
\end{tabular}
    \caption[]{Training sparse LeNet models on MNIST.}
    \label{fig:mnist_lenet_comparison}
\end{figure}

==> latex_figs/mnist_mlp_comparison.tex <==
\begin{figure}[h!]
\setlength\tabcolsep{0pt}%
\centering
\hspace{-1.5cm}
\begin{tabular}{llccc}
 \centering
 & \hspace{2mm} & \hspace{-2mm} \textbf{$L_0$-density} & \hspace{6mm}\textbf{Parameters} & \hspace{5mm} \textbf{MACs} \\
 
\rotatebox{90}{\hspace{1.2cm} \textbf{Layer-wise}} & & \includegraphics[width=0.4\textwidth, trim={0mm 0mm 0mm 0mm}, clip]{figs/control/mnist/MLP_layerwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_params/mnist/MLP_layerwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_macs/mnist/MLP_layerwise.pdf} \\
\rotatebox{90}{\hspace{1.2cm} \textbf{Model-wise}} &  & \includegraphics[width=0.4\textwidth, trim={0mm 0mm 0mm 0mm}, clip]{figs/control/mnist/MLP_modelwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_params/mnist/MLP_modelwise.pdf}
 & \includegraphics[width=0.32\textwidth]{figs/error_vs_macs/mnist/MLP_modelwise.pdf} \\
\end{tabular}
    \caption[]{Training sparse MLP models on MNIST.}
    \label{fig:mnist_mlp_comparison}
\end{figure}

==> latex_figs/stable_training.tex <==
\begin{figure}[h]
\vspace{-2ex}
\setlength\tabcolsep{2pt}%
\centering
\begin{tabular}{cc}
 \centering
%
%
\includegraphics[width=0.37\textwidth]{figs/stable_training/L0ResNet18_modelwise.pdf} & \includegraphics[width=0.48\textwidth]{figs/stable_training/ResNet-28-10_layerwise.pdf} \\
\end{tabular}
    \vspace{-2ex}
    \caption[]{Density levels for a ResNet18 (trained with a model-wise constraint) and the last sparsifiable layer of a WideResNet-28-10 model (trained with layer-wise constraints).}
    \label{fig:stable_training}
\end{figure}

==> latex_figs/tiny_imagenet_comparison.tex <==
\begin{figure}[h]
\vspace{-8ex}
\setlength\tabcolsep{0pt}%
\centering
\begin{tabular}{llccc}
 \centering
 & \hspace{2mm} & \hspace{-2mm} \textbf{$L_0$-density} & \hspace{6mm}\textbf{Parameters} & \hspace{5mm} \textbf{MACs} \\
 
\rotatebox{90}{\hspace{1.3cm} \textbf{Layer-wise}} & & \includegraphics[width=0.345\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/control/tiny_imagenet/L0ResNet18_layerwise.pdf}
 & \includegraphics[width=0.27\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/error_vs_params/tiny_imagenet/L0ResNet18_layerwise.pdf}
 & \includegraphics[width=0.27\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/error_vs_macs/tiny_imagenet/L0ResNet18_layerwise.pdf} \\
\rotatebox{90}{\hspace{1.3cm} \textbf{Model-wise}} &  & \includegraphics[width=0.345\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/control/tiny_imagenet/L0ResNet18_modelwise.pdf}
 & \includegraphics[width=0.27\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/error_vs_params/tiny_imagenet/L0ResNet18_modelwise.pdf}
 & \includegraphics[width=0.27\textwidth, trim={0mm 2mm 0mm 2mm}, clip]{figs/error_vs_macs/tiny_imagenet/L0ResNet18_modelwise.pdf}
\end{tabular}
    \vspace{-1ex}
    \caption[]{Training sparse ResNet18 models on TinyImageNet \citep{tinyImagenet}. Density denotes the proportion of active gates in the model. The penalty-based method (red) shows a stagnating-then-overshooting behavior, making it difficult to tune. In contrast, our proposed constrained approach (blue) reliably achieves the desired target $L_0$-densities. The diagonal denotes the ideal case in which the achieved density exactly matches the target density used in the constrained setting. Parameters and MACs are computed for the corresponding \textit{purged} networks following the procedure described in \cref{app:purging_models}.}
    \label{fig:tiny_imagenet_comparison}
\end{figure}

==> tables/cifar100_control.tex <==
\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.1}


\caption{Achieved density levels and performance for sparse WideResNet-28-10 models trained on CIFAR-100 for 200 epochs. Metrics aggregated over 5 runs.}
\label{tab:cifar100_control}
\vspace{1ex}

\resizebox{\textwidth}{!}{%
    
\begin{tabular}{llccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Hyper-params}} & \multirow{2}{*}{$L_0$-\textbf{density} (\%)} & \multirow{2}{*}{\textbf{Params} (\%)} & \multirow{2}{*}{\textbf{MACs} (\%)} & \multicolumn{2}{c}{\textbf{Val. Error } (\%)} \\
 & & & & & best & at 200 epochs \\
\hline
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ $g \in [1:12]$ \\ {\color{gray} \textit{Layer-wise}}}}& $\epsilon_g = 20 \%$ & $20.20 {\color{gray} \, \pm 0.00}$ & $16.94 {\color{gray} \, \pm 0.06}$ & $16.30 {\color{gray} \, \pm 0.08}$ & 20.67 & $21.07 {\color{gray} \, \pm 0.19}$ \\
& $\epsilon_g = 35 \%$ & $35.03 {\color{gray} \, \pm 0.02}$ & $31.97 {\color{gray} \, \pm 0.14}$ & $31.27 {\color{gray} \, \pm 0.08}$ & 19.71 & $20.26 {\color{gray} \, \pm 0.37}$ \\
& $\epsilon_g = 50 \%$ & $49.97 {\color{gray} \, \pm 0.03}$ & $47.30 {\color{gray} \, \pm 0.31}$ & $46.87 {\color{gray} \, \pm 0.31}$ & 19.58 & $19.87 {\color{gray} \, \pm 0.21}$ \\
& $\epsilon_g = 65 \%$ & $64.99 {\color{gray} \, \pm 0.02}$ & $63.11 {\color{gray} \, \pm 0.05}$ & $63.01 {\color{gray} \, \pm 0.17}$ & 18.89 & $19.37 {\color{gray} \, \pm 0.27}$ \\
& $\epsilon_g = 80 \%$ & $79.82 {\color{gray} \, \pm 0.15}$ & $79.33 {\color{gray} \, \pm 0.30}$ & $79.29 {\color{gray} \, \pm 0.43}$ & 18.93 & $19.32 {\color{gray} \, \pm 0.21}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ $g \in [1:12]$ \\ {\color{gray} \textit{Layer-wise}}}}  & $\lambda_{pen}^g = 1$ & \multicolumn{5}{c}{\color{gray}{------ \;\;\; \textit{Failed \; due \; to \; sparsity \; collapse}} \;\;\; ------ } \\
& $\lambda_{pen}^g = 0.1$ & $30.80 {\color{gray} \, \pm 0.54}$ & $28.63 {\color{gray} \, \pm 0.52}$ & $19.30 {\color{gray} \, \pm 0.20}$ & 20.40 & $20.89 {\color{gray} \, \pm 0.29}$ \\
& $\lambda_{pen}^g = 0.01$ & $74.46 {\color{gray} \, \pm 0.41}$ & $73.90 {\color{gray} \, \pm 0.39}$ & $59.69 {\color{gray} \, \pm 0.36}$ & 19.03 & $19.52 {\color{gray} \, \pm 0.15}$ \\
& $\lambda_{pen}^g = 0.001$ & $89.38 {\color{gray} \, \pm 0.12}$ & $89.31 {\color{gray} \, \pm 0.17}$ & $87.42 {\color{gray} \, \pm 0.40}$ & 18.72 & $19.15 {\color{gray} \, \pm 0.33}$ \\
& $\lambda_{pen}^g = 0.0001$ & $90.55 {\color{gray} \, \pm 0.34}$ & $90.74 {\color{gray} \, \pm 0.34}$ & $89.81 {\color{gray} \, \pm 0.42}$ & 18.67 & $18.96 {\color{gray} \, \pm 0.22}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ {\color{gray} \textit{Model-wise}}}} & $\epsilon = 20 \%$ & $21.50 {\color{gray} \, \pm 0.19}$ & $20.10 {\color{gray} \, \pm 0.29}$ & $24.72 {\color{gray} \, \pm 0.31}$ & 20.42 & $20.81 {\color{gray} \, \pm 0.07}$ \\
& $\epsilon = 35 \%$ & $35.46 {\color{gray} \, \pm 0.01}$ & $34.82 {\color{gray} \, \pm 0.11}$ & $44.46 {\color{gray} \, \pm 0.76}$ & 19.29 & $19.88 {\color{gray} \, \pm 0.16}$ \\
& $\epsilon = 50 \%$ & $50.16 {\color{gray} \, \pm 0.01}$ & $49.63 {\color{gray} \, \pm 0.09}$ & $60.54 {\color{gray} \, \pm 0.88}$ & 19.25 & $19.65 {\color{gray} \, \pm 0.17}$ \\
& $\epsilon = 65 \%$ & $65.08 {\color{gray} \, \pm 0.04}$ & $64.64 {\color{gray} \, \pm 0.14}$ & $72.20 {\color{gray} \, \pm 0.60}$ & 18.86 & $19.22 {\color{gray} \, \pm 0.25}$ \\
& $\epsilon = 80 \%$ & $80.12 {\color{gray} \, \pm 0.03}$ & $79.82 {\color{gray} \, \pm 0.04}$ & $82.33 {\color{gray} \, \pm 0.46}$ & 18.91 & $19.16 {\color{gray} \, \pm 0.25}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ {\color{gray} \textit{Model-wise}}}} & $\lambda_{pen} = 1 $ & $22.37 {\color{gray} \, \pm 0.39}$ & $21.07 {\color{gray} \, \pm 0.48}$ & $28.49 {\color{gray} \, \pm 0.62}$ & 20.34 & $20.79 {\color{gray} \, \pm 0.32}$ \\ 
& $\lambda_{pen} = 0.1 $ & $71.90 {\color{gray} \, \pm 0.73}$ & $71.66 {\color{gray} \, \pm 0.71}$ & $74.22 {\color{gray} \, \pm 0.43}$ & 18.37 & $18.83 {\color{gray} \, \pm 0.47}$ \\
& $\lambda_{pen} = 0.01 $ & $88.65 {\color{gray} \, \pm 0.73}$ & $88.60 {\color{gray} \, \pm 0.80}$ & $88.39 {\color{gray} \, \pm 0.83}$ & 18.41 & $18.99 {\color{gray} \, \pm 0.37}$ \\
& $\lambda_{pen} = 0.001 $ & $90.46 {\color{gray} \, \pm 0.23}$ & $90.53 {\color{gray} \, \pm 0.45}$ & $90.06 {\color{gray} \, \pm 0.62}$ & 18.75 & $19.22 {\color{gray} \, \pm 0.16}$ \\
& $\lambda_{pen} = 0.0001 $ & $90.70 {\color{gray} \, \pm 0.33}$ & $90.83 {\color{gray} \, \pm 0.35}$ & $90.03 {\color{gray} \, \pm 0.32}$ & 19.02 & $19.42 {\color{gray} \, \pm 0.10}$ \\
\hline
\end{tabular}

}

\end{table}

%


==> tables/cifar100_table.tex <==
\begin{table*}[h]

    \caption{Achieved density levels and performance for sparse WideResNets-28-10 models trained on CIFAR-100 for 200 epochs. Metrics aggregated over 5 runs. {\small $^\dag$Result reported by \citet{louizos2017learning}, with $N$ denoting the training set size (see \cref{app:normalized_l0}).}}
    \label{tab:cifar100}
    \vspace{1ex}

    %
    \renewcommand{\arraystretch}{1.1}
    %
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{clcccccc}
      \hline
      \multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{Hyper-params}} & \multirow{3}{*}{$\eta_{\text{primal}}^{\vphi}$}  & \multirow{3}{*}{$L_0$-\textbf{density} (\%)} & \multirow{3}{*}{\textbf{Params} (\%)} & \multirow{3}{*}{\textbf{MACs} (\%)} & \multicolumn{2}{c}{\textbf{Val. Error} (\%)}  \\
      \cline{7-8} & & & & & & \multirow{2}{*}{best} & at 200 epochs \\
       & & & & & & & (avg {\color{gray} $\pm$ 95\% CI)}\\
      \hline
      \hline
       \multirow{5}{*}{Penalized} & $^\dag\lambda_{pen} = 0.001/N$ & 0.1 & \multicolumn{1}{c}{\textbf{--}} &  \multicolumn{1}{c}{\textbf{--}} &  \multicolumn{1}{c}{\textbf{--}} &  \multicolumn{1}{c}{${18.75}$} & \multicolumn{1}{c}{\textbf{--}} \\
       & $^\dag\lambda_{pen} = 0.002/N$ & 0.1 & \multicolumn{1}{c}{\textbf{--}} & \multicolumn{1}{c}{\textbf{--}} &  \multicolumn{1}{c}{\textbf{--}} & \multicolumn{1}{c}{${19.04}$} & \multicolumn{1}{c}{\textbf{--}} \\
       \cline{2-8}
       & $\lambda_{pen} = 0.001$ & 0.1 & $93.20 {\color{gray} \, \pm 0.01}$ & $100.00 {\color{gray} \, \pm 0.00}$ & $100.00 {\color{gray} \, \pm 0.00}$ & $21.01$ & $21.70 {\color{gray} \, \pm 0.19}$ \\
       & $\lambda_{pen} = 0.001$ & 6 & $90.64 {\color{gray} \, \pm 0.32}$ & $90.88 {\color{gray} \, \pm 0.41}$ & $89.94 {\color{gray} \, \pm 0.71}$ & $18.51$ & $19.14 {\color{gray} \, \pm 0.21}$ \\
       & $\lambda_{pen} = 0.002$ & 6 & $90.13 {\color{gray} \, \pm 0.45}$ & $90.19 {\color{gray} \, \pm 0.38}$ & $89.52 {\color{gray} \, \pm 0.57}$ & $18.99$ & $19.24 {\color{gray} \, \pm 0.14}$ \\
       \cline{1-8}
       \multirow{2}{*}{Constrained} & $\epsilon_g = 100\%$ & 0.1 & $93.20 {\color{gray} \, \pm 0.01}$ & $100.00 {\color{gray} \, \pm 0.00}$ & $100.00 {\color{gray} \, \pm 0.00}$ & $21.02$ & $21.66 {\color{gray} \, \pm 0.21}$  \\
       \scriptsize \multirow{2}{*}{$g \in [1:12]$} & $\epsilon_g = 100 \%$ & 6 & $90.77 {\color{gray} \, \pm 0.31}$ & $90.99 {\color{gray} \, \pm 0.25}$ & $89.74 {\color{gray} \, \pm 0.29}$ & $18.68$ & $19.08 {\color{gray} \, \pm 0.16}$\\
       & $\epsilon_g = 70\%$ & 6 & $69.99 {\color{gray} \, \pm 0.01}$ & $68.62 {\color{gray} \, \pm 0.08}$ & $68.59 {\color{gray} \, \pm 0.22}$ & $18.88$ & $19.37 {\color{gray} \, \pm 0.15}$ \\
       \hline
    \end{tabular}
    }
\end{table*}


==> tables/cifar10_control.tex <==
\begin{table}[h!]
\centering

\caption{Achieved density levels and performance for sparse WideResNet-28-10 models trained on CIFAR-10 for 200 epochs. Metrics aggregated over 5 runs.}
\label{tab:cifar10_control}
\vspace{1ex}

\resizebox{\textwidth}{!}{%
    
\begin{tabular}{llccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Hyper-params}} & \multirow{2}{*}{$L_0$-\textbf{density} (\%)} & \multirow{2}{*}{\textbf{Params} (\%)} & \multirow{2}{*}{\textbf{MACs} (\%)} & \multicolumn{2}{c}{\textbf{Val. Error } (\%)} \\
 & & & & & best & at 200 epochs \\
\hline
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ $g \in [1:12]$ \\ {\color{gray} \textit{Layer-wise}}}} & $\epsilon_g = 20 \%$ & $20.00 {\color{gray} \, \pm 0.02}$ & $16.24 {\color{gray} \, \pm 0.20}$ & $16.10 {\color{gray} \, \pm 0.23}$ & 4.05 & $4.28 {\color{gray} \, \pm 0.16}$ \\
& $\epsilon_g = 35 \%$ & $34.99 {\color{gray} \, \pm 0.01}$ & $30.80 {\color{gray} \, \pm 0.34}$ & $31.05 {\color{gray} \, \pm 0.23}$ & 3.8 & $4.13 {\color{gray} \, \pm 0.13}$ \\
& $\epsilon_g = 50 \%$ & $50.00 {\color{gray} \, \pm 0.01}$ & $46.54 {\color{gray} \, \pm 0.21}$ & $46.79 {\color{gray} \, \pm 0.28}$ & 3.87 & $4.12 {\color{gray} \, \pm 0.21}$ \\
& $\epsilon_g = 65 \%$ & $64.99 {\color{gray} \, \pm 0.01}$ & $63.74 {\color{gray} \, \pm 0.33}$ & $63.63 {\color{gray} \, \pm 0.27}$ & 3.7 & $4.02 {\color{gray} \, \pm 0.11}$ \\
& $\epsilon_g = 80 \%$ & $80.00 {\color{gray} \, \pm 0.00}$ & $82.10 {\color{gray} \, \pm 0.32}$ & $81.60 {\color{gray} \, \pm 0.34}$ & 3.69 & $3.96 {\color{gray} \, \pm 0.15}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ $g \in [1:12]$ \\ {\color{gray} \textit{Layer-wise}}}}
& $\lambda_{pen}^g = 1$ & \multicolumn{5}{c}{\color{gray}{------ \;\;\; \textit{Failed \; due \; to \; sparsity \; collapse}} \;\;\; ------ } \\
& $\lambda_{pen}^g = 0.1$ & $16.09 {\color{gray} \, \pm 0.14}$ & $13.43 {\color{gray} \, \pm 0.11}$ & $11.54 {\color{gray} \, \pm 0.29}$ & 4.23 & $4.56 {\color{gray} \, \pm 0.09}$ \\
& $\lambda_{pen}^g = 0.01$ & $61.83 {\color{gray} \, \pm 0.86}$ & $62.10 {\color{gray} \, \pm 0.97}$ & $50.91 {\color{gray} \, \pm 0.62}$ & 3.83 & $4.05 {\color{gray} \, \pm 0.02}$ \\
& $\lambda_{pen}^g = 0.001$ & $89.81 {\color{gray} \, \pm 0.06}$ & $92.55 {\color{gray} \, \pm 0.13}$ & $88.91 {\color{gray} \, \pm 0.15}$ & 3.7 & $3.93 {\color{gray} \, \pm 0.15}$ \\
& $\lambda_{pen}^g = 0.0001$ & $91.54 {\color{gray} \, \pm 0.33}$ & $94.41 {\color{gray} \, \pm 0.48}$ & $92.18 {\color{gray} \, \pm 0.94}$ & 3.81 & $4.03 {\color{gray} \, \pm 0.05}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ {\color{gray} \textit{Model-wise}}}} & $\epsilon = 20 \%$ & $20.22 {\color{gray} \, \pm 0.01}$ & $18.91 {\color{gray} \, \pm 0.03}$ & $35.62 {\color{gray} \, \pm 0.84}$ & 3.95 & $4.35 {\color{gray} \, \pm 0.25}$ \\
& $\epsilon = 35 \%$  & $35.07 {\color{gray} \, \pm 0.03}$ & $34.55 {\color{gray} \, \pm 0.08}$ & $55.87 {\color{gray} \, \pm 1.23}$ & 3.76 & $4.13 {\color{gray} \, \pm 0.27}$ \\
& $\epsilon = 50 \%$ & $50.00 {\color{gray} \, \pm 0.01}$ & $49.21 {\color{gray} \, \pm 0.33}$ & $67.53 {\color{gray} \, \pm 0.08}$ & 3.79 & $4.02 {\color{gray} \, \pm 0.06}$ \\
& $\epsilon = 65 \%$ & $65.01 {\color{gray} \, \pm 0.01}$ & $64.65 {\color{gray} \, \pm 0.34}$ & $77.02 {\color{gray} \, \pm 0.43}$ & 3.80  & $3.99 {\color{gray} \, \pm 0.14}$ \\
& $\epsilon = 80 \%$ & $80.01 {\color{gray} \, \pm 0.00}$ & $81.96 {\color{gray} \, \pm 0.12}$ & $85.11 {\color{gray} \, \pm 0.58}$ & 3.83 & $3.93 {\color{gray} \, \pm 0.09}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ {\color{gray} \textit{Model-wise}}}} & $\lambda_{pen} = 1$ & $14.07 {\color{gray} \, \pm 0.23}$ & $12.09 {\color{gray} \, \pm 0.24}$ & $21.92 {\color{gray} \, \pm 0.59}$ & 4.23 & $4.43 {\color{gray} \, \pm 0.10}$ \\
& $\lambda_{pen} = 0.1$ & $48.08 {\color{gray} \, \pm 2.05}$ & $48.50 {\color{gray} \, \pm 2.27}$ & $64.58 {\color{gray} \, \pm 1.57}$ & 3.87 & $4.02 {\color{gray} \, \pm 0.22}$ \\
& $\lambda_{pen} = 0.01$ & $88.89 {\color{gray} \, \pm 0.31}$ & $91.85 {\color{gray} \, \pm 0.47}$ & $90.76 {\color{gray} \, \pm 0.77}$ & 3.72 & $3.90 {\color{gray} \, \pm 0.18}$ \\
& $\lambda_{pen} = 0.001$ & $91.24 {\color{gray} \, \pm 0.20}$ & $94.17 {\color{gray} \, \pm 0.24}$ & $92.34 {\color{gray} \, \pm 0.22}$ & 3.59 & $3.84 {\color{gray} \, \pm 0.25}$ \\
& $\lambda_{pen} = 0.0001$ & $91.98 {\color{gray} \, \pm 0.42}$ & $94.75 {\color{gray} \, \pm 0.31}$ & $92.68 {\color{gray} \, \pm 0.36}$ & 3.91 & $4.13 {\color{gray} \, \pm 0.09}$ \\
\hline
\end{tabular}
}
\end{table}


==> tables/cifar10_table.tex <==
\begin{table*}[h!]

    \caption{Achieved density levels and performance for sparse WideResNets-28-10 models trained on CIFAR-10 for 200 epochs. Metrics aggregated over 5 runs. {\small $^\dag$Result reported by \citet{louizos2017learning}, with $N$ denoting the training set size (see \cref{app:normalized_l0}).}}
    \label{tab:cifar10}
    \vspace{1ex}

    %
    \renewcommand{\arraystretch}{1.1}
    %
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{clccccccc}
      \hline
      \multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{Hyper-params}} & \multirow{3}{*}{$\eta_{\text{primal}}^{\vphi}$}  & \multirow{3}{*}{$L_0$-\textbf{density} (\%)} & \multirow{3}{*}{\textbf{Params} (\%)} & \multirow{3}{*}{\textbf{MACs} (\%)} & \multicolumn{2}{c}{\textbf{Val. Error} (\%)}  \\
      \cline{7-8} & & & & & & \multirow{2}{*}{best} & at 200 epochs \\
       & & & & & & & (avg {\color{gray} $\pm$ 95\% CI)}\\
      \hline
       \multirow{5}{*}{Penalized} & $^\dag\lambda_{pen} = 0.001/N$ & 0.1 & \multicolumn{1}{c}{\textbf{--}} &  \multicolumn{1}{c}{\textbf{--}} &  \multicolumn{1}{c}{\textbf{--}} &  \multicolumn{1}{c}{${3.83}$} & \multicolumn{1}{c}{\textbf{--}} \\
       & $^\dag\lambda_{pen} = 0.002/N$ & 0.1 & \multicolumn{1}{c}{\textbf{--}} & \multicolumn{1}{c}{\textbf{--}} &  \multicolumn{1}{c}{\textbf{--}} & \multicolumn{1}{c}{${3.93}$} & \multicolumn{1}{c}{\textbf{--}} \\
       \cline{2-8}
       & $\lambda_{pen} = 0.001$ & 0.1 & $92.30 {\color{gray} \, \pm 0.01}$ & $99.84 {\color{gray} \, \pm 0.00}$ & $100 {\color{gray} \, \pm 0.00}$ & $4.23$ & $4.56 {\color{gray} \, \pm 0.18}$ \\
       & $\lambda_{pen} = 0.001$ & 6 & $91.19 {\color{gray} \, \pm 0.16}$ & $93.98 {\color{gray} \, \pm 0.24}$ & $91.57 {\color{gray} \, \pm 0.35}$ & $3.75$ & $4.04 {\color{gray} \, \pm 0.15}$ \\
       & $\lambda_{pen} = 0.002$ & 6 & $91.36 {\color{gray} \, \pm 0.11}$ & $94.26 {\color{gray} \, \pm 0.22}$ & $92.10 {\color{gray} \, \pm 0.46}$ & $3.62$ & $4.05 {\color{gray} \, \pm 0.14}$ \\
       \cline{1-8}
       \multirow{2}{*}{Constrained} & $\epsilon_g = 100\%$ & 0.1 & $92.34 {\color{gray} \, \pm 0.01}$ & $99.84 {\color{gray} \, \pm 0.00}$ & $100 {\color{gray} \, \pm 0.00}$ & $4.18$ & $4.63 {\color{gray} \, \pm 0.14}$ \\
       \scriptsize \multirow{2}{*}{$g \in [1:12]$} & $\epsilon_g = 100 \%$ & 6 & $91.63 {\color{gray} \, \pm 0.27}$ & $94.52 {\color{gray} \, \pm 0.26}$ & $92.75 {\color{gray} \, \pm 0.58}$ & $3.74$ & $4.12 {\color{gray} \, \pm 0.08}$ \\
       & $\epsilon_g = 70\%$ & 6 & $70.00 {\color{gray} \, \pm 0.00}$ & $69.87 {\color{gray} \, \pm 0.20}$ & $69.55 {\color{gray} \, \pm 0.17}$ & $3.76$ & $4.10 {\color{gray} \, \pm 0.16}$ \\
       \hline
    \end{tabular}
    }
\end{table*}


==> tables/constrained_imagenet.tex <==
\begin{table}[ht]
\small
\centering
%

\caption{Layerwise ImageNet ResNet50}
\label{tab:imagenet_table}
\vspace{1ex}

%
\begin{tabular}{ccccc}
\hline
 \textbf{Target Density} & $L_0$-\textbf{density} (\%) & \textbf{Params} (\%) & \textbf{MACs} (\%) & \textbf{Val. Error} (\%) \\
\hline
\hline
 Baseline  & $100$  & [25.5M]  & [$4.12 \cdot 10^9$]  & $23.90$ \\
$\epsilon_g = 90 \%$  & $90.51$  & $88.00$  & $86.98$  & $26.56$ \\
$\epsilon_g = 80 \%$  & $80.54$  & $74.39$  & $72.69$  & $27.86$ \\
$\epsilon_g = 70 \%$  & $70.73$  & $61.09$  & $57.72$  & $27.81$ \\
\hline
\end{tabular}
%
\end{table}

==> tables/lenet_control.tex <==
\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.1}


\caption{Achieved density levels and performance for sparse LeNet models trained on MNIST for 200 epochs. Metrics aggregated over 5 runs.}
\label{tab:lenet_control}
\vspace{1ex}

\resizebox{\textwidth}{!}{%
    
\begin{tabular}{clccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Hyper-params}} & \multirow{2}{*}{$L_0$-\textbf{density} (\%)} & \multirow{2}{*}{\textbf{Params} (\%)} & \multirow{2}{*}{\textbf{MACs} (\%)} & \multicolumn{2}{c}{\textbf{Val. Error } (\%)} \\
 & & & & & best & at 200 epochs \\
\hline
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ $g \in [1:4]$ \\ {\color{gray} \textit{Layer-wise}}}}& $\epsilon_g = 20 \%$ & $20.09  {\color{gray} \, \pm 0.07}$ & $2.36 {\color{gray} \, \pm 0.14}$ & $4.68  {\color{gray} \,  \pm 0.68}$ & 0.81 & $1.20 {\color{gray} \, \pm 0.08}$ \\
& $\epsilon_g = 35 \%$ & $35.01 {\color{gray} \, \pm 0.01}$ & $8.59 {\color{gray} \, \pm 0.03}$ & $11.65 {\color{gray} \, \pm 1.15}$ & 0.69 & $0.84 {\color{gray} \, \pm 0.08}$ \\
& $\epsilon_g = 50 \%$ & $50.02 {\color{gray} \, \pm 0.01}$ & $21.38 {\color{gray} \, \pm 0.77}$ & $24.03 {\color{gray} \, \pm 1.64}$ & 0.56 & $0.69 {\color{gray} \, \pm 0.07}$ \\
& $\epsilon_g = 65 \%$ & $65.02 {\color{gray} \, \pm 0.01}$ & $44.01 {\color{gray} \, \pm 2.16}$ & $43.38 {\color{gray} \, \pm 2.39}$ & 0.53 & $0.65 {\color{gray} \, \pm 0.09}$ \\
& $\epsilon_g = 80 \%$ & $80.04 {\color{gray} \, \pm 0.02}$ & $76.62 {\color{gray} \, \pm 0.99}$ & $68.83  {\color{gray} \, \pm 1.40}$  & 0.45 & $0.60 {\color{gray} \, \pm 0.04}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ $g \in [1:4]$ \\ {\color{gray} \textit{Layer-wise}}}}  & $\lambda_{pen}^g = 1$ & $14.58 {\color{gray} \, \pm 0.44}$ & $0.67 {\color{gray} \, \pm 0.13}$ & $2.60 {\color{gray} \, \pm 0.17}$ & 0.46 & $1.7 {\color{gray} \, \pm 0.14}$ \\
& $\lambda_{pen}^g = 0.1$ & $37.38 {\color{gray} \, \pm 0.49}$ & $7.06 {\color{gray} \, \pm 0.36}$ & $14.62 {\color{gray} \, \pm 1.68}$ & 0.54 & $0.85 {\color{gray} \, \pm 0.02}$ \\
& $\lambda_{pen}^g = 0.01$ & $90.63 {\color{gray} \, \pm 0.20}$ & $96.43 {\color{gray} \, \pm 0.83}$ & $88.52 {\color{gray} \, \pm 7.17}$ & 0.40 & $0.56 {\color{gray} \, \pm 0.03}$ \\
& $\lambda_{pen}^g = 0.001$ & $92.77 {\color{gray} \, \pm 0.06}$ & $99.75 {\color{gray} \, \pm 0.12}$ & $99.95 {\color{gray} \, \pm 0.02}$ & 0.47 & $0.60 {\color{gray} \, \pm 0.05}$ \\
& $\lambda_{pen}^g = 0.0001$ & $92.96 {\color{gray} \, \pm 0.04}$ & $99.87 {\color{gray} \, \pm 0.12}$ & $99.98 {\color{gray} \, \pm 0.02}$ & 0.47 & $0.64 {\color{gray} \, \pm 0.06}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ {\color{gray} \textit{Model-wise}}}} & $\epsilon = 20 \%$ & $20.27 {\color{gray} \, \pm 0.30}$ & $16.58 {\color{gray} \, \pm 0.73}$ & $73.67 {\color{gray} \, \pm 0.14}$ & 0.54 & $0.85 {\color{gray} \, \pm 0.09}$ \\
& $\epsilon = 35 \%$ & $35.06 {\color{gray} \, \pm 0.09}$ & $31.36 {\color{gray} \, \pm 0.27}$ & $85.47 {\color{gray} \, \pm 0.85}$ & 0.55 & $0.71 {\color{gray} \, \pm 0.03}$ \\
& $\epsilon = 50 \%$ & $50.58 {\color{gray} \, \pm 0.09}$ & $49.41 {\color{gray} \, \pm 0.29}$ & $90.18 {\color{gray} \, \pm 0.94}$ & 0.44 & $0.64 {\color{gray} \, \pm 0.03}$ \\
& $\epsilon = 65 \%$ & $65.47 {\color{gray} \, \pm 0.05}$ & $69.60 {\color{gray} \, \pm 1.06}$ & $94.37 {\color{gray} \, \pm 0.20}$  & 0.44 & $0.72 {\color{gray} \, \pm 0.03}$ \\
& $\epsilon = 80 \%$ & $80.36 {\color{gray} \, \pm 0.08}$ & $91.86 {\color{gray} \, \pm 0.79}$ & $98.49 {\color{gray} \, \pm 0.15}$ & 0.46 & $0.58 {\color{gray} \, \pm 0.03}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ {\color{gray} \textit{Model-wise}}}} & $\lambda_{pen} = 1 $ & $13.01 {\color{gray} \, \pm 0.81}$ & $8.79  {\color{gray} \, \pm 0.80}$  & $50.47 {\color{gray} \, \pm 4.74}$ & 0.71 & $0.92 {\color{gray} \, \pm 0.11}$ \\
& $\lambda_{pen} = 0.1 $  & $42.25 {\color{gray} \, \pm 0.83}$ & $41.03 {\color{gray} \, \pm 1.12}$ & $89.08 {\color{gray} \, \pm 0.21}$ & 0.45 & $0.74 {\color{gray} \, \pm 0.04}$ \\
& $\lambda_{pen} = 0.01 $  & $90.78 {\color{gray} \, \pm 0.20}$ & $99.78 {\color{gray} \, \pm 0.20}$ & $99.96 {\color{gray} \, \pm 0.04}$ & 0.44 & $0.63 {\color{gray} \, \pm 0.05}$ \\
& $\lambda_{pen} = 0.001 $ & $92.80 {\color{gray} \, \pm 0.01}$ & $100 {\color{gray} \, \pm 0.00}$ & $100 {\color{gray} \, \pm 0.00}$ & 0.43 & $0.59 {\color{gray} \, \pm 0.01}$ \\
& $\lambda_{pen} = 0.0001 $ & $92.97 {\color{gray} \, \pm 0.03}$ & $99.94 {\color{gray} \, \pm 0.12}$ & $99.99 {\color{gray} \, \pm 0.02}$ & 0.45 & $0.59 {\color{gray} \, \pm 0.07}$ \\
\hline
\end{tabular}

}

\end{table}


==> tables/mlp_control.tex <==
\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.1}

\caption{Achieved density levels and performance for sparse MLP models trained on MNIST for 200 epochs. Metrics aggregated over 5 runs.}
\label{tab:mlp_control}
\vspace{1ex}

\resizebox{\textwidth}{!}{%
\begin{tabular}{clccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Hyper-params}} & \multirow{2}{*}{$L_0$-\textbf{density} (\%)} & \multirow{2}{*}{\textbf{Params} (\%)} & \multirow{2}{*}{\textbf{MACs} (\%)} & \multicolumn{2}{c}{\textbf{Val. Error } (\%)} \\
 & & & & & best & at 200 epochs \\
\hline
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ $g \in [1:3]$ \\ {\color{gray} \textit{Layer-wise}}}} & $\epsilon_g = 20 \%$  & $23.28 {\color{gray} \, \pm 0.31}$  & $3.41 {\color{gray} \, \pm 0.16}$  & $3.43 {\color{gray} \, \pm 0.16}$  & 1.65 & $2.82 {\color{gray} \, \pm 0.31}$ \\
& $\epsilon_g = 35 \%$  & $36.02 {\color{gray} \, \pm 0.08}$  & $10.59 {\color{gray} \, \pm 0.17}$  & $10.62 {\color{gray} \, \pm 0.17}$  & 1.66 & $2.03 {\color{gray} \, \pm 0.13}$ \\
& $\epsilon_g = 50 \%$  & $50.42 {\color{gray} \, \pm 0.04}$  & $23.60 {\color{gray} \, \pm 0.14}$  & $23.63 {\color{gray} \, \pm 0.14}$  & 1.58 & $1.76 {\color{gray} \, \pm 0.15}$ \\
& $\epsilon_g = 65 \%$  & $65.07 {\color{gray} \, \pm 0.03}$  & $42.43 {\color{gray} \, \pm 0.51}$  & $42.46 {\color{gray} \, \pm 0.51}$  & 1.42 & $1.72 {\color{gray} \, \pm 0.01}$ \\
& $\epsilon_g = 80 \%$  & $80.08 {\color{gray} \, \pm 0.07}$  & $65.53 {\color{gray} \, \pm 0.76}$  & $65.55 {\color{gray} \, \pm 0.76}$  & 1.38 & $1.54 {\color{gray} \, \pm 0.05}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ $g \in [1:3]$ \\ {\color{gray} \textit{Layer-wise}}}}  & $\lambda_{pen}^g = 1$  & $28.16 {\color{gray} \, \pm 0.97}$  & $3.58 {\color{gray} \, \pm 0.51}$  & $3.60 {\color{gray} \, \pm 0.51}$  & 2.62 & $2.93 {\color{gray} \, \pm 0.09}$ \\
 & $\lambda_{pen}^g = 0.1$  & $59.97 {\color{gray} \, \pm 0.09}$  & $33.29 {\color{gray} \, \pm 0.06}$  & $33.32 {\color{gray} \, \pm 0.06}$  & 1.37 & $1.83 {\color{gray} \, \pm 0.07}$ \\
& $\lambda_{pen}^g = 0.01$  & $90.18 {\color{gray} \, \pm 0.22}$  & $99.15 {\color{gray} \, \pm 0.94}$  & $99.15 {\color{gray} \, \pm 0.94}$  & 1.29 & $1.44 {\color{gray} \, \pm 0.13}$ \\
& $\lambda_{pen}^g = 0.001$  & $93.77 {\color{gray} \, \pm 0.10}$  & $99.23 {\color{gray} \, \pm 0.22}$  & $99.23 {\color{gray} \, \pm 0.22}$  & 1.33 & $1.60  {\color{gray} \, \pm 0.10}$  \\
& $\lambda_{pen}^g = 0.0001$  & $94.04 {\color{gray} \, \pm 0.23}$  & $99.67 {\color{gray} \, \pm 0.38}$  & $99.67 {\color{gray} \, \pm 0.38}$  & 1.26 & $1.51 {\color{gray} \, \pm 0.04}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ {\color{gray} \textit{Model-wise}}}} & $\epsilon = 20 \%$  & $22.77 {\color{gray} \, \pm 0.17}$  & $12.80 {\color{gray} \, \pm 0.41}$  & $12.87 {\color{gray} \, \pm 0.41}$  & 1.40  & $2.11 {\color{gray} \, \pm 0.05}$ \\
& $\epsilon = 35 \%$  & $36.25 {\color{gray} \, \pm 0.06}$  & $30.07 {\color{gray} \, \pm 0.39}$  & $30.16 {\color{gray} \, \pm 0.39}$  & 1.37 & $1.75 {\color{gray} \, \pm 0.11}$ \\
& $\epsilon = 50 \%$  & $50.89 {\color{gray} \, \pm 0.12}$  & $49.71 {\color{gray} \, \pm 0.27}$  & $49.78 {\color{gray} \, \pm 0.27}$  & 1.20 & $1.46 {\color{gray} \, \pm 0.16}$ \\
& $\epsilon = 65 \%$  & $65.37 {\color{gray} \, \pm 0.01}$  & $65.57 {\color{gray} \, \pm 0.22}$  & $65.62 {\color{gray} \, \pm 0.22}$  & 1.27 & $1.50 {\color{gray} \, \pm 0.03}$ \\
& $\epsilon = 80 \%$  & $80.02 {\color{gray} \, \pm 0.05}$  & $77.08 {\color{gray} \, \pm 0.86}$  & $77.11 {\color{gray} \, \pm 0.86}$  & 1.16 & $1.46 {\color{gray} \, \pm 0.16}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ {\color{gray} \textit{Model-wise}}}} & $\lambda_{pen} = 1 $  & $27.73 {\color{gray} \, \pm 0.15}$  & $18.54 {\color{gray} \, \pm 0.51}$  & $18.62 {\color{gray} \, \pm 0.52}$  & 1.48 & $1.91 {\color{gray} \, \pm 0.07}$ \\
& $\lambda_{pen} = 0.1 $  & $62.38 {\color{gray} \, \pm 0.16}$  & $62.37 {\color{gray} \, \pm 0.3}$  & $62.43 {\color{gray} \, \pm 0.3}$  & 1.30 & $1.53 {\color{gray} \, \pm 0.13}$ \\
& $\lambda_{pen} = 0.01$  & $90.98 {\color{gray} \, \pm 0.18}$  & $99.56 {\color{gray} \, \pm 0.43}$  & $99.56 {\color{gray} \, \pm 0.43}$  & 1.34 & $1.51 {\color{gray} \, \pm 0.11}$ \\
& $\lambda_{pen} = 0.001 $  & $93.81 {\color{gray} \, \pm 0.17}$  & $99.89 {\color{gray} \, \pm 0.22}$  & $99.89 {\color{gray} \, \pm 0.22}$  & 1.24 & $1.57 {\color{gray} \, \pm 0.09}$ \\
& $\lambda_{pen} = 0.0001$  & $93.99 {\color{gray} \, \pm 0.06}$  & $99.67 {\color{gray} \, \pm 0.38}$  & $99.67 {\color{gray} \, \pm 0.38}$  & 1.32 & $1.60 {\color{gray} \, \pm 0.17}$ \\
\hline
\end{tabular}
}
\end{table}

==> tables/mnist_table.tex <==
\begin{table*}[ht]
    %
    \renewcommand{\arraystretch}{1.05}
    \centering
    %
    
    \caption{Achieved density levels and performance for sparse MLP and LeNet5 models     trained on MNIST for 200 epochs. Metrics aggregated over 5 runs. {\small $^\dag$Results by \citet{louizos2017learning} with $N$ representing the training set size (see \cref{app:normalized_l0}).}
    }
    \label{tab:mnist}
    %

    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ccclccc}
      \hline
      \multirow{3}{*}{\textbf{Architecture}} & \multirow{3}{*}{\textbf{Grouping}} & \multirow{3}{*}{\textbf{Method}}  & \multirow{3}{*}{\textbf{\hspace{5mm}Hyper-parameters}} & \textbf{Pruned} & \multicolumn{2}{c}{\textbf{Val. Error} (\%)}  \\
      \cline{6-7} & & &  &  \multirow{2}{*}{\textbf{architecture}} & \multirow{2}{*}{best} & at 200 epochs \\
       & & & & &  & (avg {\color{gray} $\pm$ 95\% CI)}\\
      \hline
      \hline
       & \multirow{2}{*}{Model} & Pen.  &  $^\dag\lambda_{pen} = 0.1/N$ &  219-214-100 & 1.4 & --\\
       MLP & & Const. &  $\epsilon = 33 \%$ &  198-233-100 & 1.36 & 1.77 {\color{gray} $\pm$ 0.08}\\
       \cline{2-7}
       784-300-100 & \multirow{2}{*}{Layer} & Pen. &  $^\dag\lambda_{pen} = [0.1,0.1,0.1]/N$ &  266-88-33 & 1.8 & -- \\
      & & Const. &  $\epsilon = [30 \%, 30\%, 30\%]$ &  243-89-29 & 1.58 & 2.19 {\color{gray} $\pm$ 0.12 }\\
       \hline
       & \multirow{2}{*}{Model} & Pen. &   $^\dag\lambda_{pen} = 0.1/N$ &  20-25-45-462 & 0.9 & --\\
       LeNet5 & & Const. &  $\epsilon = 10\%$ &  20-21-34-407 & 0.56 & 1.01 {\color{gray} $\pm$ 0.05}\\
       \cline{2-7}
       20-50-800-500 & \multirow{2}{*}{Layer} & Pen. &  $^\dag\lambda_{pen} = [10,0.5,0.1,0.1]/N$ &  9-18-65-25 & 1.0 & -- \\
       & & Const. &  $\epsilon = [50\%, 30\%, 70\%, 10\%]$ &  10-14-224-29 & 0.7 & 0.91 {\color{gray} $\pm$ 0.05}\\
       \hline
    \end{tabular}
    } %

\end{table*}

==> tables/mp_comparison_imagenet.tex <==
\begin{table}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.0}

\caption{Layer-wise pruning of ResNet50 models on ImageNet.}
\label{tab:mp_comparison_imagenet}
\vspace{1ex}

%
\begin{tabular}{cccccc}
\hline
\textbf{Target Density} & \textbf{Method} & $L_0$-\textbf{density} (\%) & \textbf{Params} (\%) & \textbf{MACs} (\%) & \textbf{Val. Error} (\%) \\
\hline
\hline
  Baseline & -  & $100$  & [25.5M]  & [$4.12 \cdot 10^9$]  & $23.90$ \\
 \hline
\multirow{2}{*}{$\epsilon_g = 90 \%$} & Constrained & $90.51$  & $88.00$  & $86.98$  & $26.56$ \\
 & L1 - Mag. Prune & - & 85.94 & 84.99 & 38.74 \\
\hline
\multirow{2}{*}{$\epsilon_g = 80 \%$} & Constrained & $80.54$  & $74.39$  & $72.69$  & $27.86$ \\
& L1 - Mag. Prune & - & 73.35 & 71.69 & 77.69\\
\hline
\multirow{2}{*}{$\epsilon_g = 70 \%$} & Constrained & $70.73$  & $61.09$  & $57.72$  & $27.81$ \\
& L1 - Mag. Prune & - & 62.15 & 59.85 & 97.78\\
\hline
\end{tabular}
%
\end{table}

==> tables/tiny_imagenet_control.tex <==
\begin{table}[h!]

\centering
\renewcommand{\arraystretch}{1.1}

\caption{Achieved density levels and performance for sparse ResNet18 models trained on TinyImageNet for 200 epochs. Metrics aggregated over 5 runs.}
\vspace{1ex}

\resizebox{\textwidth}{!}{%
    
%
\begin{tabular}{llllllllllll}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Hyper-params}} & \multirow{2}{*}{$L_0$-\textbf{density} (\%)} & \multirow{2}{*}{\textbf{Params} (\%)} & \multirow{2}{*}{\textbf{MACs} (\%)} & \multicolumn{2}{c}{\textbf{Val. Error } (\%)} \\
 & & & & & best & at 200 epochs \\
\hline
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ $g \in [1:16]$ \\ {\color{gray} \textit{Layer-wise}}}} & $\epsilon_g = 20 \%$ & $23.88 {\color{gray} \, \pm 0.72}$ & $12.01 {\color{gray} \, \pm 0.42}$ & $10.62 {\color{gray} \, \pm 0.35}$ & 46.94 & $47.80 {\color{gray} \, \pm 0.16}$ \\
& $\epsilon_g = 35 \%$ & $35.41 {\color{gray} \, \pm 0.07}$ & $21.16 {\color{gray} \, \pm 0.03}$ & $20.25 {\color{gray} \, \pm 0.16}$ & 43.87 & $45.16 {\color{gray} \, \pm 0.31}$ \\
& $\epsilon_g = 50 \%$ & $50.40 {\color{gray} \, \pm 0.04}$ & $34.22 {\color{gray} \, \pm 0.28}$ & $32.73 {\color{gray} \, \pm 0.49}$ & 42.52 & $43.80 {\color{gray} \, \pm 0.44}$ \\
& $\epsilon_g = 65 \%$ & $65.32 {\color{gray} \, \pm 0.42}$ & $50.22 {\color{gray} \, \pm 0.54}$ & $47.34 {\color{gray} \, \pm 0.66}$ & 41.80 & $42.61 {\color{gray} \, \pm 0.10}$ \\
& $\epsilon_g = 80 \%$ & $79.68 {\color{gray} \, \pm 0.88}$ & $68.78 {\color{gray} \, \pm 1.70}$ & $65.98 {\color{gray} \, \pm 1.53}$ & 40.55 & $41.17 {\color{gray} \, \pm 0.61}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ $g \in [1:16]$ \\ {\color{gray} \textit{Layer-wise}}}}  & $\lambda_{pen}^g = 1$ & \multicolumn{5}{c}{\color{gray}{------ \;\;\; \textit{Failed \; due \; to \; sparsity \; collapse}} \;\;\; ------ } \\
& $\lambda_{pen}^g = 0.1$ & $35.90 {\color{gray} \, \pm 0.57}$ & $18.98 {\color{gray} \, \pm 0.57}$ & $10.77 {\color{gray} \, \pm 0.90}$ & 46.34 & $48.70 {\color{gray} \, \pm 0.73}$ \\
& $\lambda_{pen}^g = 0.01$ & $78.77 {\color{gray} \, \pm 0.84}$ & $65.59 {\color{gray} \, \pm 1.94}$ & $50.66 {\color{gray} \, \pm 1.77}$ & 41.36 & $42.15 {\color{gray} \, \pm 0.27}$ \\
& $\lambda_{pen}^g = 0.001$ & $86.87 {\color{gray} \, \pm 0.38}$ & $77.14 {\color{gray} \, \pm 1.29}$ & $67.45 {\color{gray} \, \pm 3.88}$ & 40.75 & $41.23 {\color{gray} \, \pm 0.58}$ \\
& $\lambda_{pen}^g = 0.0001$ & $87.77 {\color{gray} \, \pm 0.42}$ & $78.85 {\color{gray} \, \pm 0.91}$ & $71.49 {\color{gray} \, \pm 2.36}$ & 40.32 & $40.68 {\color{gray} \, \pm 0.04}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Constrained \\ {\color{gray} \textit{Model-wise}}}} & $\epsilon = 20 \%$ & $26.26 {\color{gray} \, \pm 0.33}$ & $14.55 {\color{gray} \, \pm 0.14}$ & $28.31 {\color{gray} \, \pm 0.35}$ & 42.64 & $43.61 {\color{gray} \, \pm 0.56}$ \\
& $\epsilon = 35 \%$ & $35.66 {\color{gray} \, \pm 0.12}$ & $21.25 {\color{gray} \, \pm 0.70}$ & $33.88 {\color{gray} \, \pm 1.25}$ & 41.28 & $42.99 {\color{gray} \, \pm 0.81}$ \\
& $\epsilon = 50 \%$ & $50.53 {\color{gray} \, \pm 0.09}$ & $33.19 {\color{gray} \, \pm 0.08}$ & $43.65 {\color{gray} \, \pm 0.94}$ & 40.70 & $42.29 {\color{gray} \, \pm 0.17}$ \\
& $\epsilon = 65 \%$ & $65.46 {\color{gray} \, \pm 0.19}$ & $49.34 {\color{gray} \, \pm 0.55}$ & $53.92 {\color{gray} \, \pm 0.97}$ & 41.23 & $41.86 {\color{gray} \, \pm 0.54}$ \\
& $\epsilon = 80 \%$ & $80.45 {\color{gray} \, \pm 0.19}$ & $67.45 {\color{gray} \, \pm 0.67}$ & $64.80 {\color{gray} \, \pm 1.18}$ & 40.71 & $41.16 {\color{gray} \, \pm 0.28}$ \\
\hline
\multirow{5}{*}{\shortstack[l]{Penalized \\ {\color{gray} \textit{Model-wise}}}} & $\lambda_{pen} = 1$ & \multicolumn{5}{c}{\color{gray}{------ \;\;\; \textit{Failed \; due \; to \; sparsity \; collapse}} \;\;\; ------ } \\
& $\lambda_{pen} = 0.1$ & $73.64 {\color{gray} \, \pm 0.72}$ & $59.27 {\color{gray} \, \pm 0.76}$ & $59.33 {\color{gray} \, \pm 2.19}$ & 40.84 & $41.69 {\color{gray} \, \pm 0.16}$ \\
& $\lambda_{pen} = 0.01$ & $83.80 {\color{gray} \, \pm 0.08}$ & $72.41 {\color{gray} \, \pm 0.67}$ & $66.64 {\color{gray} \, \pm 1.26}$ & 40.33 & $41.29 {\color{gray} \, \pm 0.50}$ \\
& $\lambda_{pen} = 0.001$ & $85.12 {\color{gray} \, \pm 0.89}$ & $74.31 {\color{gray} \, \pm 1.72}$ & $67.30 {\color{gray} \, \pm 1.62}$ & 40.71 & $41.28 {\color{gray} \, \pm 0.56}$ \\
& $\lambda_{pen} = 0.0001$ & $84.84 {\color{gray} \, \pm 0.90}$ & $73.80 {\color{gray} \, \pm 1.53}$ & $66.91 {\color{gray} \, \pm 1.65}$ & 40.57 & $41.05 {\color{gray} \, \pm 0.33}$ \\
\hline
\end{tabular}

}
\end{table}

%

